The second data release from the European Pulsar Timing Array: IV. Implications for massive black holes, dark matter and the early Universe

The European Pulsar Timing Array (EPTA) and Indian Pulsar Timing Array (InPTA) collaborations have measured a low-frequency common signal in the combination of their second and first data releases respectively, with the correlation properties of a gravitational wave background (GWB). Such signal may have its origin in a number of physical processes including a cosmic population of inspiralling supermassive black hole binaries (SMBHBs); inflation, phase transitions, cosmic strings and tensor mode generation by non-linear evolution of scalar perturbations in the early Universe; oscillations of the Galactic potential in the presence of ultra-light dark matter (ULDM). At the current stage of emerging evidence, it is impossible to discriminate among the different origins. Therefore, in this paper, we consider each process separately, and investigate the implications of the signal under the hypothesis that it is generated by that specific process. We find that the signal is consistent with a cosmic population of inspiralling SMBHBs, and its relatively high amplitude can be used to place constraints on binary merger timescales and the SMBH-host galaxy scaling relations. If this origin is confirmed, this is the first direct evidence that SMBHBs merge in nature, adding an important observational piece to the puzzle of structure formation and galaxy evolution. As for early Universe processes, the measurement would place tight constraints on the cosmic string tension and on the level of turbulence developed by first-order phase transitions. Other processes would require non-standard scenarios, such as a blue-tilted inflationary spectrum or an excess in the primordial spectrum of scalar perturbations at large wavenumbers. Finally, a ULDM origin of the detected signal is disfavoured, which leads to direct constraints on the abundance of ULDM in our Galaxy.

==> acknowledgements_alt.tex <==
The European Pulsar Timing Array (EPTA) is a collaboration between
European and partner institutes, namely ASTRON (NL), INAF/Osservatorio
di Cagliari (IT), Max-Planck-Institut f\"{u}r Radioastronomie (GER),
Nan\c{c}ay/Paris Observatory (FRA), the University of Manchester (UK),
the University of Birmingham (UK), the University of East Anglia (UK),
the University of Bielefeld (GER), the University of Paris (FRA), the
University of Milan-Bicocca (IT), the Foundation for Research and 
Technology, Hellas (GR), and Peking University (CHN), with the
aim to provide high-precision pulsar timing to work towards the direct
detection of low-frequency gravitational waves. An Advanced Grant of
the European Research Council allowed to implement the Large European Array
for Pulsars (LEAP) under Grant Agreement Number 227947 (PI M. Kramer). 
The EPTA is part of the
International Pulsar Timing Array (IPTA); we thank our
IPTA colleagues for their support and help with this paper and the external Detection Committee members for their work on the Detection Checklist.

Part of this work is based on observations with the 100-m telescope of
the Max-Planck-Institut f\"{u}r Radioastronomie (MPIfR) at Effelsberg
in Germany. Pulsar research at the Jodrell Bank Centre for
Astrophysics and the observations using the Lovell Telescope are
supported by a Consolidated Grant (ST/T000414/1) from the UK's Science
and Technology Facilities Council (STFC). ICN is also supported by the
STFC doctoral training grant ST/T506291/1. The Nan{\c c}ay radio
Observatory is operated by the Paris Observatory, associated with the
French Centre National de la Recherche Scientifique (CNRS), and
partially supported by the Region Centre in France. We acknowledge
financial support from ``Programme National de Cosmologie and
Galaxies'' (PNCG), and ``Programme National Hautes Energies'' (PNHE)
funded by CNRS/INSU-IN2P3-INP, CEA and CNES, France. We acknowledge
financial support from Agence Nationale de la Recherche
(ANR-18-CE31-0015), France. The Westerbork Synthesis Radio Telescope
is operated by the Netherlands Institute for Radio Astronomy (ASTRON)
with support from the Netherlands Foundation for Scientific Research
(NWO). The Sardinia Radio Telescope (SRT) is funded by the Department
of University and Research (MIUR), the Italian Space Agency (ASI), and
the Autonomous Region of Sardinia (RAS) and is operated as a National
Facility by the National Institute for Astrophysics (INAF).

The work is supported by the National SKA programme of China
(2020SKA0120100), Max-Planck Partner Group, NSFC 11690024, CAS
Cultivation Project for FAST Scientific. This work is also supported
as part of the ``LEGACY'' MPG-CAS collaboration on low-frequency
gravitational wave astronomy. JA acknowledges support from the
European Commission (Grant Agreement number: 101094354). JA and SCha 
were partially supported by the Stavros
Niarchos Foundation (SNF) and the Hellenic Foundation for Research and
Innovation (H.F.R.I.) under the 2nd Call of the ``Science and Society --
Action Always strive for excellence -- Theodoros Papazoglou''
(Project Number: 01431). AC acknowledges support from the Paris
\^{I}le-de-France Region. AC, AF, ASe, ASa, EB, DI, GMS, MBo acknowledge
financial support provided under the European Union's H2020 ERC
Consolidator Grant ``Binary Massive Black Hole Astrophysics'' (B
Massive, Grant Agreement: 818691). GD, KLi, RK and MK acknowledge support
from European Research Council (ERC) Synergy Grant ``BlackHoleCam'', 
Grant Agreement Number 610058. This work is supported by the ERC 
Advanced Grant ``LEAP'', Grant Agreement Number 227947 (PI M. Kramer). 
AV and PRB are supported by the UK's Science
and Technology Facilities Council (STFC; grant ST/W000946/1). AV also acknowledges
the support of the Royal Society and Wolfson Foundation. JPWV acknowledges
support by the Deutsche Forschungsgemeinschaft (DFG) through thew
Heisenberg programme (Project No. 433075039) and by the NSF through
AccelNet award \#2114721. NKP is funded by the Deutsche
Forschungsgemeinschaft (DFG, German Research Foundation) --
Projektnummer PO 2758/1--1, through the Walter--Benjamin
programme. ASa thanks the Alexander von Humboldt foundation in
Germany for a Humboldt fellowship for postdoctoral researchers. APo, DP
and MBu acknowledge support from the research grant “iPeska”
(P.I. Andrea Possenti) funded under the INAF national call
Prin-SKA/CTA approved with the Presidential Decree 70/2016
(Italy). RNC acknowledges financial support from the Special Account
for Research Funds of the Hellenic Open University (ELKE-HOU) under
the research programme ``GRAVPUL'' (grant agreement 319/10-10-2022).
EvdW, CGB and GHJ acknowledge support from the Dutch National Science
Agenda, NWA Startimpuls – 400.17.608.
BG is supported by the Italian Ministry of Education, University and 
Research within the PRIN 2017 Research Program Framework, n. 2017SYRTCN. LS acknowledges the use of the HPC system Cobra at the Max Planck Computing and Data Facility.

\ifnum\wm>1 The Indian Pulsar Timing Array (InPTA) is an Indo-Japanese
collaboration that routinely employs TIFR's upgraded Giant Metrewave
Radio Telescope for monitoring a set of IPTA pulsars.  BCJ, YG, YM,
SD, AG and PR acknowledge the support of the Department of Atomic
Energy, Government of India, under Project Identification \# RTI 4002.
BCJ, YG and YM acknowledge support of the Department of Atomic Energy,
Government of India, under project No. 12-R\&D-TFR-5.02-0700 while SD,
AG and PR acknowledge support of the Department of Atomic Energy,
Government of India, under project no. 12-R\&D-TFR-5.02-0200.  KT is
partially supported by JSPS KAKENHI Grant Numbers 20H00180, 21H01130,
and 21H04467, Bilateral Joint Research Projects of JSPS, and the ISM
Cooperative Research Program (2021-ISMCRP-2017). AS is supported by
the NANOGrav NSF Physics Frontiers Center (awards \#1430284 and
2020265).  AKP is supported by CSIR fellowship Grant number
09/0079(15784)/2022-EMR-I.  SH is supported by JSPS KAKENHI Grant
Number 20J20509.  KN is supported by the Birla Institute of Technology
\& Science Institute fellowship.  AmS is supported by CSIR fellowship
Grant number 09/1001(12656)/2021-EMR-I and T-641 (DST-ICPS).  TK is
partially supported by the JSPS Overseas Challenge Program for Young
Researchers.  We acknowledge the National Supercomputing Mission (NSM)
for providing computing resources of ‘PARAM Ganga’ at the Indian
Institute of Technology Roorkee as well as `PARAM Seva' at IIT
Hyderabad, which is implemented by C-DAC and supported by the Ministry
of Electronics and Information Technology (MeitY) and Department of
Science and Technology (DST), Government of India. DD acknowledges the 
support from the Department of Atomic Energy, Government of India 
through Apex Project - Advance Research and Education in Mathematical 
Sciences at IMSc. \fi


The work presented here is a culmination of many years of data
analysis as well as software and instrument development. In particular,
we thank Drs. N.~D'Amico, P.~C.~C.~Freire, R.~van Haasteren, 
C.~Jordan, K.~Lazaridis, P.~Lazarus, L.~Lentati, O.~L\"{o}hmer and 
R.~Smits for their past contributions. We also
thank Dr. N. Wex for supporting the calculations of the
galactic acceleration as well as the related discussions. We would like to thank Prof. Drs. Alexey Starobinskiy, Sergei Blinnikov and Alexander Dolgov for discussions on the early Universe physics.
The EPTA is also grateful
to staff at its observatories and telescopes who have made the
continued observations possible. 

==> authorlist_alt.tex <==
%% Authornames here:
%% Check list of labels in institute.tex or at the bottom of this file.
%% Please fix the numbers!
\author{J.~Antoniadis\orcidlink{0000-0003-4453-776}\inst{\ref{forth},\ref{mpifr}},
        P.~Auclair\orcidlink{0000-0002-4814-1406}\inst{\ref{curl}},
		S.~Babak\orcidlink{0000-0001-7469-4250}\inst{\ref{apc}},
		A.-S.~Bak~Nielsen\orcidlink{ 0000-0002-1298-9392}\inst{\ref{mpifr}\ref{unibi}},
        E.~Barausse\orcidlink{0000-0001-6499-6263 }\inst{\ref{sissa}},
		C.~G.~Bassa\orcidlink{0000-0002-1429-9010}\inst{\ref{astron}},
		A.~Berthereau\inst{\ref{lpc2e},\ref{nancay}},
		M.~Bonetti\orcidlink{0000-0001-7889-6810}\inst{\ref{unimib},\ref{infn-unimib},\ref{inaf-brera}},
        E.~Bortolas\inst{\ref{unimib},\ref{infn-unimib},\ref{inaf-brera}},
        P.~R.~Brook\orcidlink{0000-0003-3053-6538}\inst{\ref{unibir}},
        M.~Burgay\orcidlink{0000-0002-8265-4344}\inst{\ref{inaf-oac}},
		R.~N.~Caballero\orcidlink{0000-0001-9084-9427}\inst{\ref{HOU}},
            C.~Caprini\orcidlink{0000-0001-5393-2205}\inst{\ref{unige},\ref{CERN}},
		A.~Chalumeau\orcidlink{0000-0003-2111-1001}\inst{\ref{unimib}}\ifnum\wm=2\thanks{aurelien.chalumeau@unimib.it}\fi,
		D.~J.~Champion\orcidlink{0000-0003-1361-7723}\inst{\ref{mpifr}},
        S.~Chanlaridis\orcidlink{0000-0002-9323-9728}\inst{\ref{forth}},
		S.~Chen\orcidlink{0000-0002-3118-5963}\inst{19}\ifnum\wm=3\thanks{sychen@pku.edu.cn}\fi,
		I.~Cognard\orcidlink{0000-0002-1775-9692}\inst{\ref{lpc2e},\ref{nancay}},
        M.~Crisostomi\orcidlink{0000-0002-7622-4911}\inst{\ref{sissa}},
		G.~Desvignes\orcidlink{0000-0003-3922-4055}\inst{\ref{mpifr}},
        F.~Fastidio\inst{\ref{surrey}, \ref{unimib}, \ref{infn-unimib}, \ref{inaf-brera}}
		M.~Falxa\inst{\ref{apc},\ref{lpc2e}}
		R.~D.~Ferdman\inst{\ref{uea}},
        A.~Franchini\inst{\ref{unimib},\ref{infn-unimib}},
		%% P.~C.~C.~Freire\inst{\ref{mpifr}},
		J.~R.~Gair\orcidlink{0000-0002-1671-3668}\inst{\ref{aei}},
        B.~Goncharov\inst{\ref{gssi},\ref{lngs}}
		E.~Graikou\inst{\ref{mpifr}},
        A.~Gualandris\orcidlink{0000-0002-9420-2679}\inst{\ref{surrey}},
        J.-M.~Grie{\ss}meier\orcidlink{0000-0003-3362-7996}\inst{\ref{lpc2e},\ref{nancay}},
		L.~Guillemot\orcidlink{0000-0002-9049-8716}\inst{\ref{lpc2e},\ref{nancay}},
		Y.~J.~Guo\inst{\ref{mpifr}}\ifnum\wm=3\thanks{yjguo@mpifr-bonn.mpg.de}\fi,
		H.~Hu\orcidlink{0000-0002-3407-8071}\inst{\ref{mpifr}}, 
        F. Iraci\inst{\ref{unica}\ref{inaf-oac}},
		D.~Izquierdo-Villalba\orcidlink{0000-0002-6143-1491}\inst{\ref{unimib},\ref{infn-unimib}},
        J.~Jang\orcidlink{0000-0003-4454-0204}\inst{\ref{mpifr}}\ifnum\wm=1\thanks{jjang@mpifr-bonn.mpg.de}\fi,
        J.~Jawor\orcidlink{0000-0003-3391-0011}\inst{\ref{mpifr}},
		G.~H.~Janssen\orcidlink{0000-0003-3068-3677}\inst{\ref{astron},\ref{imapp}},
		R.~Karuppusamy\orcidlink{0000-0002-5307-2919}\inst{\ref{mpifr}},
        E.~F.~Keane\orcidlink{0000-0002-4553-655X}\inst{\ref{tcd}},
		M.~J.~Keith\orcidlink{0000-0001-5567-5492}\inst{\ref{jbca}}\ifnum\wm=2\thanks{michael.keith@manchester.ac.uk}\fi,
          T.~Khizriev,\inst{\ref{SAI}},
		M.~Kramer\inst{\ref{mpifr},\ref{jbca}},
        M.~A.~Krishnakumar\orcidlink{0000-0003-4528-2745}\inst{\ref{mpifr},\ref{unibi}},
        K.~Lackeos\orcidlink{0000-0002-6554-3722}\inst{\ref{mpifr}},
		K.~J.~Lee\inst{3,8,\ref{mpifr}},
		K.~Liu\inst{\ref{mpifr}}\ifnum\wm=1\thanks{kliu@mpifr-bonn.mpg.de}\fi,
        Y.~Liu\orcidlink{0000-0001-9986-9360}\inst{\ref{naoc}, \ref{unibi}},
		%% X.~J.~Liu\inst{20,\ref{jbca}},
		A.~G.~Lyne\inst{\ref{jbca}},
		J.~W.~McKee\orcidlink{0000-0002-2885-8485}\inst{\ref{milne},\ref{daim}},
		R.~A.~Main\inst{\ref{mpifr}},
		M.~B.~Mickaliger\orcidlink{0000-0001-6798-5682}\inst{\ref{jbca}},H.~Middleton\orcidlink{0000-0001-5532-3622}\inst{\ref{unibir}},
        A.~Neronov\inst{\ref{apc}, \ref{EPFL}},
        I.~C.~Ni\c{t}u\orcidlink{0000-0003-3611-3464}\inst{\ref{jbca}},
		A.~Parthasarathy\orcidlink{0000-0002-4140-5616}\inst{\ref{mpifr}}\ifnum\wm=2\thanks{aparthas@mpifr-bonn.mpg.de}\fi,
		B.~B.~P.~Perera\inst{\ref{arecibo}},
		D.~Perrodin\orcidlink{0000-0002-1806-2483}\inst{\ref{inaf-oac}},
		A.~Petiteau\orcidlink{0000-0002-7371-9695}\inst{\ref{irfu},\ref{apc}},
		N.~K.~Porayko\inst{\ref{unimib}, \ref{mpifr}},
		A.~Possenti\inst{\ref{inaf-oac}},
          K.~Postnov\orcidlink{0000-0002-1705-617X}\inst{\ref{SAI}, \ref{KFU}},
		H.~Quelquejay~Leclere\inst{\ref{apc}},
            A.~Roper Pol\orcidlink{0000-0003-4979-4430}\inst{\ref{unige}},
        A.~Samajdar\orcidlink{0000-0002-0857-6018}\inst{\ref{uni-potsdam}},
		S.~A.~Sanidas\inst{\ref{jbca}},
            D.~Semikoz\inst{\ref{apc}},
		A.~Sesana\inst{\ref{unimib},\ref{infn-unimib},\ref{inaf-brera}},
		G.~Shaifullah\orcidlink{0000-0002-8452-4834}\inst{\ref{unimib},\ref{infn-unimib},\ref{inaf-oac}}\ifnum\wm=1\thanks{golam.shaifullah@unimib.it}\fi,
        C.~Smarra\inst{\ref{sissa}},
		L.~Speri\orcidlink{0000-0002-5442-7267}\inst{\ref{aei}},
        R.~Spiewak\inst{\ref{jbca}},
		B.~W.~Stappers\inst{\ref{jbca}},
        D.~A.~Steer\orcidlink{0000-0002-8781-1273}\inst{\ref{apc}}
        S.~C.~Susarla\orcidlink{0000-0003-4332-8201}\inst{\ref{uog}},
		G.~Theureau\orcidlink{0000-0002-3649-276X}\inst{\ref{lpc2e}, \ref{nancay}, \ref{luth}},
		C.~Tiburzi\inst{\ref{inaf-oac}},
        R.~J.~Truant\inst{\ref{unimib}},
        S.~Valtolina\inst{\ref{aei2}},
		E.~van~der~Wateren\orcidlink{0000-0003-0382-8463}\inst{\ref{astron},\ref{imapp}},
		A.~Vecchio\orcidlink{0000-0002-6254-1617}\inst{\ref{unibir}},
        V.~Venkatraman~Krishnan\orcidlink{0000-0001-9518-9819}\inst{\ref{mpifr}},
		J.~P.~W.~Verbiest\orcidlink{0000-0002-4088-896X}\inst{\ref{FSI},\ref{unibi},\ref{mpifr}},
	    J.~Wang\orcidlink{0000-0003-1933-6498}\inst{\ref{unibi}, \ref{airub}, \ref{bnuz}},
		L.~Wang\inst{\ref{jbca}},
        Z.~Wu\orcidlink{0000-0002-1381-7859}\inst{\ref{naoc}, \ref{unibi}},
	    %% H.~Xu\inst{3,26,8},
        P.~Arumugam\orcidlink{0000-0001-9264-8024}\inst{\ref{IITR}},
        S.~Arumugam\orcidlink{0009-0001-3587-6622}\inst{\ref{IITH_El}},
        M.~Bagchi\orcidlink{0000-0001-8640-8186}\inst{\ref{IMSc},\ref{HBNI}},
        A.~Bathula\orcidlink{0000-0001-7947-6703} \inst{\ref{IISERM}},
        S.~Dandapat\orcidlink{0000-0003-4965-9220}\inst{\ref{TIFR}},
        S.~Desai\orcidlink{0000-0002-0466-3288}\inst{\ref{IITH_Ph}},
        N.~Dhanda-Batra \inst{\ref{UoD}},
        C.~Dwivedi\orcidlink{0000-0002-8804-650X}\inst{\ref{IIST}},
        A.~Gopakumar\orcidlink{0000-0003-4274-4369}\inst{\ref{TIFR}},
        Y.~Gupta\orcidlink{0000-0001-5765-0619}\inst{\ref{NCRA}},
        S.~Hisano\orcidlink{0000-0002-7700-3379}\inst{\ref{KU_J}},
        B.~C.~Joshi\orcidlink{0000-0002-0863-7781}\inst{\ref{NCRA},\ref{IITR}},
        F.~Kareem\orcidlink{0000-0003-2444-838X} \inst{\ref{IISERK},\ref{CESSI}},
        D.~Kharbanda\orcidlink{0000-0001-8863-4152}\inst{\ref{IITH_Ph}},
        T.~Kikunaga\orcidlink{0000-0002-5016-3567} \inst{\ref{KU_J}},
        N.~Kolhe\orcidlink{0000-0003-3528-9863} \inst{\ref{XCM}},
        Y.~Maan\inst{\ref{NCRA}},
        K.~Nobleson\orcidlink{0000-0003-2715-4504}\inst{\ref{BITS}},
        A.~K.~Paladi\orcidlink{0000-0002-8651-9510}\inst{\ref{IISc}},
        T.~Prabu\inst{\ref{RRI}},
        P.~Rana\orcidlink{0000-0001-6184-5195}\inst{\ref{TIFR}},
        J.~Singha\orcidlink{0000-0002-1636-9414}\inst{\ref{IITR}},
        A.~Srivastava\orcidlink{0000-0003-3531-7887} \inst{\ref{IITH_Ph}},
        M.~Surnis\orcidlink{0000-0002-9507-6985}\inst{\ref{IISERB}},
        A.~Susobhanan\orcidlink{0000-0002-2820-0931}\inst{\ref{CGCA}},
        K.~Takahashi\orcidlink{0000-0002-3034-5769}\inst{\ref{KU_J1},\ref{KU_J2}}, and
        P.~Tarafdar\orcidlink{0000-0001-6921-4195}\inst{\ref{IMSc}}
        }

%%% institute labels here
% \label{forth}
% \label{mpifr}
% \label{arecibo}
% \label{aia}
% \label{astron}
% \label{cita}
% \label{imapp}
% \label{unimib}
% \label{unibi}
% \label{inaf-oac}
% \label{infn-unimib}
% \label{unibir}
% \label{jbca}
% \label{kiaa}
% \label{lpc2e}
% \label{luth}
% \label{lesia}
% \label{aei}
% \label{mipt}
% \label{naoc}
% \label{uea}
% \label{nancay}
% \label{unica}
% \label{apc}
% \label{uni-potsdam}

==> institutes_alt.tex <==
%% Institutes here
%% Numbers are 2(n+1) of the lines number on the side
\institute{
ASTRON, Netherlands Institute for Radio Astronomy, Oude Hoogeveensedijk 4, 7991 PD, Dwingeloo, The Netherlands\label{astron}\and
Advanced Institute of Natural Sciences, Beijing Normal University, Zhuhai 519087, China \label{bnuz}\and
Arecibo Observatory, HC3 Box 53995, Arecibo, PR 00612, USA\label{arecibo}\and
Canadian Institute for Theoretical Astrophysics, University of Toronto, 60 St. George Street, Toronto, ON M5S 3H8, Canada\label{cita}\and
Center for Gravitation, Cosmology, and Astrophysics, University of Wisconsin-Milwaukee, Milwaukee, WI 53211, USA \label{CGCA}\and
Centre of Excellence for Data Science, Artificial Intelligence and Modelling (DAIM), University of Hull, Cottingham Road, Kingston-upon-Hull, HU6 7RX, UK\label{daim}\and
Department of Astrophysics/IMAPP, Radboud University Nijmegen, P.O. Box 9010, 6500 GL Nijmegen, The Netherlands\label{imapp}\and
Dipartimento di Fisica ``G. Occhialini", Universit{\'a} degli Studi di Milano-Bicocca, Piazza della Scienza 3, I-20126 Milano, Italy\label{unimib}\and
Kazan Federal University, 18 Kremlyovskaya, 420008 Kazan, Russia\label{KFU}\and
E.A. Milne Centre for Astrophysics, University of Hull, Cottingham Road, Kingston-upon-Hull, HU6 7RX, UK\label{milne}\and
Fakult{\"a}t f{\"u}r Physik, Universit{\"a}t Bielefeld, Postfach 100131, 33501 Bielefeld, Germany\label{unibi}\and
Florida Space Institute, University of Central Florida, 12354 Research Parkway, Partnership 1 Building, Suite 214, Orlando, 32826-0650, FL, USA\label{FSI}\and
Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy \label{gssi}\and
Hellenic Open University, School of Science and Technology, 26335 Patras, Greece\label{HOU}\and
INAF - Osservatorio Astronomico di Brera, via Brera 20, I-20121 Milano, Italy\label{inaf-brera}\and
INAF - Osservatorio Astronomico di Cagliari, via della Scienza 5, 09047 Selargius (CA), Italy\label{inaf-oac}\and
INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy \label{lngs}\and 
IRFU, CEA, Université Paris-Saclay, F-91191 Gif-sur-Yvette, France \label{irfu}\and
INFN, Sezione di Milano-Bicocca, Piazza della Scienza 3, I-20126 Milano, Italy\label{infn-unimib}\and
Institut f\"{u}r Physik und Astronomie, Universit\"{a}t Potsdam, Haus 28, Karl-Liebknecht-Str. 24/25, 14476, Potsdam, Germany\label{uni-potsdam}\and
Institute for Gravitational Wave Astronomy and School of Physics and Astronomy, University of Birmingham, Edgbaston, Birmingham B15 2TT, UK\label{unibir}\and
Institute of Astrophysics, FORTH, N. Plastira 100, 70013, Heraklion, Greece\label{forth}\and 
Jodrell Bank Centre for Astrophysics, Department of Physics and Astronomy, University of Manchester, Manchester M13 9PL, UK\label{jbca}\and
Kavli Institute for Astronomy and Astrophysics, Peking University, Beijing 100871, P. R. China\label{kiaa}\and
Laboratoire Univers et Th{\'e}ories LUTh, Observatoire de Paris, Universit{\'e} PSL, CNRS, Universit{\'e} de Paris, 92190 Meudon, France\label{luth}\and
Laboratoire de Physique et Chimie de l'Environnement et de l'Espace, Universit\'e d'Orl\'eans / CNRS, 45071 Orl\'eans Cedex 02, France \label{lpc2e}\and
Max Planck Institute for Gravitational Physics (Albert Einstein Institute), Am Mu{\"u}hlenberg 1, 14476 Potsdam, Germany\label{aei}\and
Max Planck Institute for Gravitational Physics (Albert
Einstein Institute), Leibniz Universit\"at Hannover, Callinstrasse 38,
D-30167, Hannover, Germany\label{aei2}\and
Max-Planck-Institut f{\"u}r Radioastronomie, Auf dem H{\"u}gel 69, 53121 Bonn, Germany\label{mpifr}\and
Sternberg Astronomical Institute, Moscow State University, Universitetsky pr., 13, Moscow 119234, Russia\label{SAI}\and
Moscow Institute of Physics and Technology, Dolgoprudny, Moscow region, Russia\label{mipt}\and
National Astronomical Observatories, Chinese Academy of Sciences, Beijing 100101, P. R. China\label{naoc}\and
Observatoire Radioastronomique de Nan\c{c}ay, Observatoire de Paris, Universit\'e PSL, Université d'Orl\'eans, CNRS, 18330 Nan\c{c}ay, France\label{nancay}\and
Ruhr University Bochum, Faculty of Physics and Astronomy, Astronomical Institute (AIRUB), 44780 Bochum, Germany \label{airub}\and
School of Mathematics and Physics, Faculty of Engineering and Physical Science, University of Surrey, Guildford GU2 7XH, UK\label{surrey}\and
School of Physics, Faculty of Science, University of East Anglia, Norwich NR4 7TJ, UK\label{uea}\and
Scuola Internazionale Superiore di Studi Avanzati: Via Bonomea 265, I-34136 Trieste, Italy and INFN Sezione di Trieste \label{sissa} \and
School of Physics, Trinity College Dublin, College Green, Dublin 2, D02 PN40, Ireland\label{tcd}\and
Ollscoil na Gaillimhe --- University of Galway, University Road, Galway, H91 TK33, Ireland\label{uog}\and
Universit{\'a} di Cagliari, Dipartimento di Fisica, S.P. Monserrato-Sestu Km 0,700 - 09042 Monserrato (CA), Italy\label{unica}\and
Universit{\'e} de Paris, CNRS, Astroparticule et Cosmologie, 75013 Paris, France\label{apc}\and
Department of Astronomy and Astrophysics, Tata Institute of Fundamental Research, Homi Bhabha Road, Navy Nagar, Colaba, Mumbai 400005, India \label{TIFR}\and
Department of Earth and Space Sciences, Indian Institute of Space Science and Technology, Valiamala, Thiruvananthapuram, Kerala 695547,India \label{IIST}\and
Department of Electrical Engineering, IIT Hyderabad, Kandi, Telangana 502284, India \label{IITH_El}\and
Department of Physical Sciences,Indian Institute of Science Education and Research Kolkata, Mohanpur, 741246, India \label{IISERK}\and
Center of Excellence in Space Sciences India, Indian Institute of Science Education and Research Kolkata, 741246, India \label{CESSI}\and 
Department of Physical Sciences, Indian Institute of Science Education and Research, Mohali, Punjab 140306, India \label{IISERM}\and
Department of Physics and Astrophysics, University of Delhi, Delhi 110007, India \label{UoD}\and
Department of Physics, BITS Pilani Hyderabad Campus, Hyderabad 500078, Telangana, India \label{BITS}\and
Department of Physics, IISER Bhopal, Bhopal Bypass Road, Bahuri, Bhopal 462066, Madhya Pradesh, India \label{IISERB}\and
Department of Physics, IIT Hyderabad, Kandi, Telangana 502284, India \label{IITH_Ph}\and
Department of Physics, Indian Institute of Technology Roorkee, Roorkee-247667, India\label{IITR}\and 
Department of Physics, St. Xavier’s College (Autonomous), Mumbai 400001, India \label{XCM}\and
Division of Natural Science, Faculty of Advanced Science and Technology, Kumamoto University, 2-39-1 Kurokami, Kumamoto 860-8555, Japan \label{KU_J1}\and
Homi Bhabha National Institute, Training School Complex, Anushakti Nagar, Mumbai 400094, India \label{HBNI}\and
International Research Organization for Advanced Science and Technology, Kumamoto University, 2-39-1 Kurokami, Kumamoto 860-8555, Japan \label{KU_J2}\and
Joint Astronomy Programme, Indian Institute of Science, Bengaluru, Karnataka, 560012, India \label{IISc}\and
Kumamoto University, Graduate School of Science and Technology, Kumamoto, 860-8555, Japan \label{KU_J}\and
National Centre for Radio Astrophysics, Pune University Campus, Pune 411007, India \label{NCRA}\and
Raman Research Institute India, Bengaluru, Karnataka, 560080, India \label{RRI}\and
The Institute of Mathematical Sciences, C. I. T. Campus, Taramani, Chennai 600113, India \label{IMSc}\and
Cosmology, Universe and Relativity at Louvain (CURL), Institute of Mathematics and Physics, University of Louvain, 2 Chemin du Cyclotron, 1348 Louvain-la-Neuve, Belgium \label{curl}\and\label{unige}Université de Gen\`eve, Département de Physique Théorique and Centre for Astroparticle Physics, 24 quai
Ernest-Ansermet, CH-1211 Genéve 4, Switzerland\and
\label{CERN}CERN, Theoretical Physics Department, 1 Esplanade des Particules, CH-1211 Genéve 23, Switzerland\and
\label{EPFL}Laboratory of Astrophysics, \'Ecole Polytechnique F\'ed\'erale de Lausanne, CH-1015 Lausanne, Switzerland
} 

==> sections/macros.tex <==
%% put your custom macros in here
\newcommand{\red}{\textcolor{red}}
\newcommand{\purple}{\textcolor{purple}}
\newcommand{\epta}[1]{{EPTA~D.R.~1}}
\newcommand{\ipta}[1]{{IPTA~D.R.~1}}
\newcommand{\mdegr}{^{\circ}}
%\newcommand{\degr}{$^{\circ}$}
\newcommand{\uppi}{\mathrm{\pi}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\iot}{\mathrm{i}}
\newcommand{\st}{\textsuperscript{st}}
\newcommand{\nd}{\textsuperscript{nd}}

\newcommand{\C}{\textsf{\textbf{C}}}
\newcommand{\Cinv}{\textsf{\textbf{C}}^{-1}}
\newcommand{\Cda}{\textsf{\textbf{C}}'}
\newcommand{\Cdainv}{\textsf{\textbf{C}}'^{-1}}

\newcommand{\Ctot}{\tilde{\textsf{\textbf{C}}}}
\newcommand{\Ctotinv}{\tilde{\textsf{\textbf{C}}}^{-1}}
\newcommand{\Ctotda}{\tilde{\textsf{\textbf{C}}}'}
\newcommand{\Ctotdainv}{\tilde{\textsf{\textbf{C}}}'^{-1}}

\newcommand{\Cpta}{\textsf{\textbf{C}}_{\rm PTA}}

\newcommand{\Cw}{\textsf{\textbf{C}}_{\textsf{W}}}
\newcommand{\Cr}{\textsf{\textbf{C}}_{\textsf{R}}}
\newcommand{\Cdm}{\textsf{\textbf{C}}_{\textsf{DM}}}
\newcommand{\Ccu}{\textsf{\textbf{C}}_{\textsf{CURN}}}
\newcommand{\Cgwb}{\textsf{\textbf{C}}_{\textsf{GWB}}}
\newcommand{\Cclk}{\textsf{\textbf{C}}_{\textsf{CLK}}}
\newcommand{\Ceph}{\textsf{\textbf{C}}_{\textsf{EPH}}}

\newcommand{\D}{\textsf{\textbf{D}}}
\newcommand{\Dtr}{\textsf{\textbf{D}}^{\textsf{T}}}
\newcommand{\Dpta}{\tilde{\textsf{\textbf{D}}}}
\newcommand{\Dptatr}{\tilde{\textsf{\textbf{D}}}^{\textsf{T}}}

\newcommand{\M}{\textsf{\textbf{M}}}
\newcommand{\Mtr}{\textsf{\textbf{M}}^{\textsf{T}}}
\newcommand{\Mpta}{\tilde{\textsf{\textbf{M}}}}
\newcommand{\Mptatr}{\tilde{\textsf{\textbf{M}}}^{\textsf{T}}}

\newcommand{\T}{\textsf{\textbf{T}}}
\newcommand{\Ttr}{\textsf{\textbf{T}}^{\textsf{T}}}
\newcommand{\B}{\textsf{\textbf{B}}}
\newcommand{\G}{\textsf{\textbf{G}}}
\newcommand{\Ginv}{\textsf{\textbf{G}}^{-1}}
\newcommand{\Gtr}{\textsf{\textbf{G}}^{\textsf{T}}}

\newcommand{\BF}{\mathcal{B}}
%_{\textrm{tot}}

\newcommand{\F}{\textsf{\textbf{F}}}
%\newcommand{\Finv}{\textsf{\textbf{F}}^{-1}}
\newcommand{\Ftr}{\textsf{\textbf{F}}^{\textsf{T}}}
\newcommand{\Fourier}{\boldsymbol{F}}
%\usepackage{pifont}
%\newcommand{\crossmark}{\ding{56}}
\newcommand{\tr}{\textsf{T}}
\newcommand{\toa}{\boldsymbol{t}}
\newcommand{\res}{\delta\boldsymbol{t}}
\newcommand{\psrsig}{\boldsymbol{\tau(\epsilon)}}
\newcommand{\crssig}{\boldsymbol{t_{\textrm{crs}}}}
\newcommand{\Acrs}{A_{\textrm{crs}}}
\newcommand{\gamcrs}{\gamma_{\textrm{crs}}}
%\newcommand{\Acrs}{A_{\textrm{crs}}}
%\newcommand{\sol}[1]{\mathrm{#1_{\odot}}}
\newcommand{\ttwo}{{\tt TEMPO2}}
\newcommand{\tn}{{\tt TEMPONEST}}
\newcommand{\mnest}{{\tt MULTINEST}}
\newcommand{\pmnest}{{\tt PYMULTINEST}}
\newcommand{\python}{{\tt PYTHON}}
\newcommand{\pchord}{{\tt POLYCHORD}}
\newcommand{\pchordlite}{{\tt POLYCHORDLITE}}
\newcommand{\psrx}{{\tt PSRCHIVE}}
\newcommand{\ftwo}{{\tt FORTYTWO}}
\newcommand{\beph}{{\tt BAYESEPHEM}}
\newcommand{\lmoss}{{\tt LINIMOSS}}
\newcommand{\egp}{{\tt EPHEMGP}}
\newcommand{\eprise}{{\tt ENTERPRISE}}
\newcommand{\ee}{{\tt ENTERPRISE\_EXTENSIONS}}
\newcommand{\ptmc}{{\tt PTMCMCSAMPLER}}
